Verifying User Interfaces using SPARK Ada: A Case Study of the T34 Syringe Driver

The increase in safety and critical systems improved Healthcare. Due to their risk of harm, such systems are subject to stringent guidelines and compliances. These safety measures ensure a seamless experience and mitigate the risk to end-users. Institutions like the Food and Drug Administration and the NHS, respectively, established international standards and competency frameworks to ensure industry compliance with these safety concerns. Medical device manufacturing is mainly concerned with standards. Consequently, these standards now advocate for better human factors considered in user interaction for medical devices. This forces manufacturers to rely on heavy testing and review to cover many of these factors during development. Sadly, many human factor risks will not be caught until proper testing in real life, which might be catastrophic in the case of an ambulatory device like the T34 syringe pump. Therefore, effort in formal methods research may propose new solutions in anticipating these errors in the early stages of development or even reducing their occurrence based on the use of standard generic model. These generically developed models will provide a common framework for safety integration in industry and may potentially be proven using formal verification mathematical proofs. This research uses SPARK Ada's formal verification tool against a behavioural model of the T34 syringe driver. A Generic Infusion Pump model refinement is explored and implemented in SPARK Ada. As a subset of the Ada language, the verification level of the end prototype is evaluated using SPARK. Exploring potential limitations defines the proposed model's implementation liability when considering abstraction and components of User Interface design in SPARK Ada.

==> Chapters/Chapter6.tex <==
% Chapter Template

\chapter{Conclusion} % Main chapter title

\label{Chapter6} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

%----------------------------------------------------------------------------------------
%	SECTION 1
%----------------------------------------------------------------------------------------

 
 

Safety-critical systems are ubiquitous today throughout people's life. Their critical role has many benefits and risks. Many examples exist, but the most contextual is the application of medical devices for patients. As benefits, we can count the lives saved in the hospital. Similarly, this benefit is associated with the high risk of these types of devices. The more these devices are adopted for many patients; the more defects are being detected. A typical device in this category is the infusion pump. Many reported incidents are related to user interface design errors that have gone unnoticed. In other cases, they are the result of confusion over the user interface display. There is, therefore, an urgent need to constantly update existing research as the number of new devices increases each year dramatically.   

 
 

In this research, the author aims to demonstrate the use of Spark Ada in user interface verification for safety-critical medical devices. The contribution of this work is the portability of safety requirements for generic infusion pumps using Spark Ada with refinement methods. At the end of this project, we hope to have a reliable prototype based on a realistic behavioural model of the T34 infusion pump. The objective is to establish a practical case study for industrial simulation or even implementation of real devices. Most importantly, it contributes to the existing body of knowledge on implementing the GIIP initiative. 
  
 [TO COMPLETE]
